Infi-MMR: Curriculum-based Unlocking Multimodal Reasoning via Phased Reinforcement Learning in Multimodal Small Language Models

Recent advancements in large language models (LLMs) have demonstrated substantial progress in reasoning capabilities, such as DeepSeek-R1, which leverages rule-based reinforcement learning to enhance logical reasoning significantly. However, extending these achievements to multimodal large language models (MLLMs) presents critical challenges, which are frequently more pronounced for Multimodal Small Language Models (MSLMs) given their typically weaker foundational reasoning abilities: (1) the scarcity of high-quality multimodal reasoning datasets, (2) the degradation of reasoning capabilities due to the integration of visual processing, and (3) the risk that direct application of reinforcement learning may produce complex yet incorrect reasoning processes. To address these challenges, we design a novel framework Infi-MMR to systematically unlock the reasoning potential of MSLMs through a curriculum of three carefully structured phases and propose our multimodal reasoning model Infi-MMR-3B. The first phase, Foundational Reasoning Activation, leverages high-quality textual reasoning datasets to activate and strengthen the model's logical reasoning capabilities. The second phase, Cross-Modal Reasoning Adaptation, utilizes caption-augmented multimodal data to facilitate the progressive transfer of reasoning skills to multimodal contexts. The third phase, Multimodal Reasoning Enhancement, employs curated, caption-free multimodal data to mitigate linguistic biases and promote robust cross-modal reasoning. Infi-MMR-3B achieves both state-of-the-art multimodal math reasoning ability (43.68% on MathVerse testmini, 27.04% on MathVision test, and 21.33% on OlympiadBench) and general reasoning ability (67.2% on MathVista testmini). Resources are available at https://huggingface.co/Reallm-Labs/Infi-MMR-3B.

==> tables/Results_on_MathVerse.tex <==
\begin{table*}[!htp]
    \centering
    \small
    % \setlength{\tabcolsep}{0pt}
    \caption{Detailed Results on MathVerse testmini. Results colored in \textcolor{Mahogany}{Mahogany} represent the best performance, and those \underline{underlined} indicate the second-best performance.}
    \label{table:mathverse}
    \resizebox{1.0\linewidth}{!}
{
    \begin{tabular}{lccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c}{\textbf{Detailed Accuracy on MathVerse testmini (\%)}} \\
    \cmidrule(lr){2-6}
    & Text Domain & Text Lite & Vision Intensive & Vision Domain & Vision Only  \\
    \midrule
    Qwen2.5-VL-3B & 43.15 & 35.41 & 33.38 & 32.87 & 28.43 \\
    InfiMMR\_FRP & 48.1 & 39.85 & 36.8 & 37.31 & 35.15  \\
    InfiMMR\_CMRA & 49.24 & 44.16 & 41.5 & 42.77 & 36.68 \\
    \textbf{InfiMMR-3B} & 51.65 &  \textcolor{Mahogany}{45.69} &  \textcolor{Mahogany}{41.12} & \textcolor{Mahogany}{42.01} & \textcolor{Mahogany}{39.97}  \\
    \bottomrule
    \end{tabular}
}
    % \vspace{-5mm}
\end{table*}
